On the Robustness of ChatGPT: An Adversarial and Out-of-distribution Perspective

ChatGPT is a recent chatbot service released by OpenAI and is receiving increasing attention over the past few months. While evaluations of various aspects of ChatGPT have been done, its robustness, i.e., the performance to unexpected inputs, is still unclear to the public. Robustness is of particular concern in responsible AI, especially for safety-critical applications. In this paper, we conduct a thorough evaluation of the robustness of ChatGPT from the adversarial and out-of-distribution (OOD) perspective. To do so, we employ the AdvGLUE and ANLI benchmarks to assess adversarial robustness and the Flipkart review and DDXPlus medical diagnosis datasets for OOD evaluation. We select several popular foundation models as baselines. Results show that ChatGPT shows consistent advantages on most adversarial and OOD classification and translation tasks. However, the absolute performance is far from perfection, which suggests that adversarial and OOD robustness remains a significant threat to foundation models. Moreover, ChatGPT shows astounding performance in understanding dialogue-related texts and we find that it tends to provide informal suggestions for medical tasks instead of definitive answers. Finally, we present in-depth discussions of possible research directions.

==> sec-append.tex <==
\section{Detailed Introduction of Datasets and Tasks}

\subsection{\advglue and ANLI}
\label{append-data-adv}

\advglue~\citep{wang2021adversarial} is an evaluation benchmark for natural language processing models, with a specific focus on adversarial robustness. It includes five natural language understanding tasks from the GLUE benchmark: Sentiment Analysis (SST-2), Duplicate Question Detection (QQP), and Natural Language Inference (NLI, including MNLI, RTE, QNLI).
It includes different types of attacks including word-level transformations, sentence-level manipulations, and human-written adversarial examples.

\textbf{SST-2} The Stanford Sentiment Treebank~\citep{socher2013recursive} is composed of sentences originating from movie reviews, along with corresponding human-annotated sentiments. The goal is to predict the sentiment (positive or negative) when given a review sentence.

\textbf{QQP} Quora Question Pairs (QQP) dataset consists of pairs of questions gathered from Quora, which is a platform for community question-answering. The aim is to predict if two questions are semantically equivalent.

\textbf{MNLI} Multi-Genre Natural Language Inference Corpus~\citep{williams2018broad} is a dataset of sentence pairs for textual entailment. The task is to predict whether the premise sentence entails, contradicts, or is neutral to the hypothesis sentence.

\textbf{QNLI} The Question-answering NLI (QNLI) dataset consists of question-sentence pairs extrated and modified from the Stanford Question Answering Dataset~\citep{rajpurkar2016squad}. The task is to predict if the context sentence has the answer to a given question.

\textbf{RTE} The Recognizing Textual Entailment (RTE) dataset contains examples constructed using news and Wikipedia text from annual textual entailment challenges. The goal is to predict the relationship between a pair of sentences, which can be categorized into two classes: entailment and not entailment. Note that neutral and contradiction are considered as not entailment.

\textbf{\advglue-T} We create an adversarial machine translation dataset (En $\to$ Zh) called \advglue-T by randomly extracting 30 samples from \advglue. 

\textbf{Adversarial NLI (ANLI)}~\citep{nie2020adversarial} is a benchmark for natural language understanding collected by using human-and-model-in-the-loop training method. This benchmark is designed to challenge the current models in natural language inference. Human annotators acted as adversaries by trying to fool the model into mis-classifying with the found vulnerabilities, while these sentences are still understandable to other humans. 


\subsection{\flip and \ddx}
\label{append-data-ood}

\flip~\citep{flipkart_2023} includes information on 104 different types of products from {\ttfamily flipkart.com}, such as electronics, clothing, home decor, and more. It contains 205,053 data and their corresponding sentiment labels (positive, negative, or neutral).
In our study, we select all its instances with review text length between $150$ and $160$ to ease the experiments.
This leads to $331$ samples in total.

\ddx~\citep{tchango2022ddxplus} is a dataset designed for automatic medical diagnosis, which consists of synthetic data of around $1.3$ million patients, providing a differential diagnosis and the true pathology, symptoms, and antecedents for each patient. We randomly sampled 100 records from the test set. As the original records were in French, we translated them into English using the evidences and conditions dictionaries provided in the dataset. The resulting data was then formatted into a context of age, gender, initial evidence, and inquiry dialogue, enabling the model to select the most probable disease from all considered pathology using the information provided in the conversation.


\section{Evaluation Metrics} \label{append-metrics-asr}
\paragraph{Attack Success Rate (ASR)} 
Following \citep{wang2021adversarial}, the metric of ASR is adopted for evaluating the effectiveness of the system against adversarial inputs. Specifically, given a dataset $\mathcal{D} = \{(x_i, y_i)\}_{i=1}^N$ consisting of $N$ samples $x_i$ and corresponding ground truth labels $y_i$, the success rate of an adversarial attack method $\mathcal{A}$, which generates adversarial examples $A(x)$ given an input $x$ to attack a surrogate model $f$, is computed as: 

\begin{equation}
\operatorname{ASR} = \sum\limits_{(x,y)\in \mathcal{D}} \frac{\mathbbm{1}[f(\mathcal{A}(x)) \neq y]}{\mathbbm{1}[f(x) = y]}
\end{equation}

Basically, the robustness of a model is inversely proportional to the attack success rate. 

\section{An Informal Analysis from the Theory Perspective}
\label{append-theory}

This section presents a brief overview of existing machine learning and robustness theory, assisting potential analysis of large foundation models.

\subsection{Machine Learning Theory}
\label{append-theory-ml}

The foundational learning theory in machine learning is called the probably approximately correct (PAC) theory~\citep{valiant1984theory}.
While our focus is to facilitate the analysis of foundation models, we only discuss the theory related to generalization error, which is the basic one.

In binary classification, we define the true labeling function $f: \mathcal{X} \rightarrow [0,1]$ for domain $\mathcal{D}$. For any classifier $h:\mathcal{X} \rightarrow [0,1]$, the classification error is defined as:
\begin{equation}
    \epsilon(h,f) = \mathbb{E}_{x \sim \mathcal{D}}[h(x) \neq f(x)] = \mathbb{E}_{x \sim \mathcal{D}}[|h(x) - f(x)|].
\end{equation}

\begin{theorem}[Generalization error]
\label{theory-generalization}
Let $\mathcal{H}$ be a finite hypothesis set, $m$ the number of training samples, and $0 < \delta < 1$, then for any $h \in \mathcal{H}$,
\begin{equation}
    P \left( |\mathbb{E}(h) - \hat{\mathbb{E}}(h)| \le \sqrt{\frac{\ln |\mathcal{H}| + \ln (2/\delta)}{2m}} \right) \ge 1 - \delta,
\end{equation}    
where $\mathbb{E}(h)$ and $\hat{\mathbb{E}}(h)$ are the ideal and empirical (learned) risk on $h$, respectively.
\end{theorem}

\cref{theory-generalization} indicates that the generalization error is determined by the number of training samples $m$ and the size of the hypothesis space $\mathcal{H}$.
The superior performance of large foundation models are typically trained on huge datasets ($m$ is large).
However, the hypothesis set $\mathcal{H}$ is finite.
Therefore, the increment of $m$ and $|\mathcal{H}|$ could lead to a lower generalization error according to \cref{theory-generalization}.
This seems to explain why large foundation models such as \chat and text-davinci-003 achieve superior performance in zero-shot classification on some tasks.
Note taht the theoretical analysis on foundation models is still underexplored, hence, this analysis could be wrong and we still look forward to theoretical advances in this area.

However, as large foundation models become more complex, it could possibly induce a high VC-dimension~\citep{valiant1984theory}.
At the same time, their training data sizes are certainly larger than existing machine learning research.
It remains unknown why such models do not overfit on existing datasets.



\subsection{Out-of-distribution Robustness Theory}
\label{append-theory-ood}

OOD assumes training on a source dataset $\mathcal{D}_s$ and test on another unseen dataset $\mathcal{D}_t$.
The key challenge is that the distributions between $\mathcal{D}_s$ and $\mathcal{D}_t$ are not the same.
Although it is impossible to evaluate the risk on an unseen dataset since we cannot even access it, we can borrow the classic domain adaptation theory to analyze the risk on the target domain by assuming its availability.

\begin{theorem}[Target error bound based on $\mathcal{H}$-divergence~\citep{ben2010theory}]
\label{theo:h}
Let $\mathcal{H}$ be a hypothesis space with VC dimension $d$. Given sample set with size $m$ i.i.d. sampled from the source domain, then, with probability at least $1-\delta$, for any $h \in \mathcal{H}$, we have:
\begin{equation}
    \epsilon_t(h) \leq \hat{\epsilon}_s(h)  + d_{\mathcal{H}}(\hat{\mathcal{D}}_s, \hat{\mathcal{D}}_t) + \lambda^\ast + \sqrt{\frac{4}{m} \left(d\log\frac{2em}{d}+\log\frac{4}{\delta} \right)},
\end{equation}
where $e$ is natural logarithm, $\lambda^\ast = \epsilon_s(h^\ast) + \epsilon_t(h^\ast)$ is the ideal joint risk, and $h^\ast = \mathop{\arg\min}\limits_{h \in \mathcal{H}} \epsilon_s(h) + \epsilon_t(h)$ is the optimal classifier on the source and target domains.
\end{theorem}

Theory \ref{theo:h} indicates that the error bound on the target domain is bounded by four terms: 1) source empirical error, 2) the distribution discrepancy between source and target domains, 3) ideal joint error, and 4) some constant related to sample size and VC dimension.

Conventional OOD generalization and adaptation research~\citep{wang2022generalizing} focus on minimizing the distribution discrepancy between source and target domains ($d_{\mathcal{H}}(\hat{\mathcal{D}}_s, \hat{\mathcal{D}}_t)$) while assuming the source risk ($\hat{\epsilon}_s(h)$) is determined.
Meanwhile, the last term ($\sqrt{\cdot}$) can also be reduced due to the increment of $m$.
Similar to the above generalization analysis, we can also interpret the success of large foundation models as they simply achieving low generalization error on the source data, thus also minimizes the risk on the target domain.
But it is also important to note that this analysis is not rigorous.
Finally, VC-dimension has no correlation with the distribution of datasets, which also cannot explain the strong OOD performance of these foundation models.

\section{Foundation Models used in Experiments}
\label{append-model}

In this section, we provide a brief introduction to the foundation models used in our experiments.

% \begin{table}[htbp]
% \centering
% \caption{Parameter and model size.}
% \label{tb-model}
% \begin{tabular}{ccc}
% \toprule
% Model            & \#Parameter & Size (GB) \\ \midrule
% BERT-L           & 335 M       & 1.3   \\ 
% RoBERTa-L        & 560 M       & 2.2   \\ 
% BART-L           & 407 M       & 1.6   \\ 
% ELECTRA-L        & 335 M       & 1.3   \\ 
% DeBERTa-L        & 435 M       & 1.7   \\ 
% GPT-2            & 1.5 B       & 3.9   \\ 
% BLOOM            & 7.1 B       & 14.1   \\ 
% OPT              & 66 B        & 131.4   \\ 
% text-davinci-002 & 175 B       & -  \\ 
% text-davinci-003 & 176 B       & -   \\ \bottomrule
% \end{tabular}
% \end{table}

% \paragraph{BERT-L~\citep{devlin2018bert}} BERT is a pre-trained language model based on the bidirectional transformer architecture. BERT obtains the ability of capturing the meaning of a word in its context by unsupervised pre-training on a large corpus using masked language modeling and next sentence prediction. After unsupervised pre-training, BERT can adapt to various down-stream tasks by being further fine-tuned down-stream data.

% \paragraph{RoBERTa-L~\citep{liu2019roberta}} RoBERTa refers to Robustly Optimized BERT approach. Compared with BERT, it uses more pre-training data, larger batch size and more training steps. Besides, RoBERTa proposes to adopt dynamic masking for masked language modeling.

\textbf{BART-L~\citep{lewis2020bart}} BART is based on bidirectional and auto-regressive transformer. It is trained on a combination of auto-regressive and denoising objectives, which makes BART feasible for both generation and understanding tasks. In a nutshell, BART is designed to handle both understanding and generation tasks, making it a more versatile model, while BERT is more focused on understanding.

% \paragraph{ELECTRA-L~\citep{clark2020electra}} In pre-training stage, ELECTRA adopts discriminative pre-training other than mask language modeling. The goal is to distinguish between real and fake tokens. The simplicity of the learning objective makes it more efficient than previous methods. 

\textbf{DeBERTa-L~\citep{he2020deberta}} DeBERTa introduces a disentangled attention mechanism and an enhanced decoding scheme for BERT. The disentangled attention mechanism allows DeBERTa to capture the contextual information between different tokens in a sentence more effectively, while the enhanced decoding scheme makes the model generate natural language sentences with higher quality. 

% \paragraph{GPT-2~\citep{radford2019language}} GPT-2 is based on a unidirectional transformer and pre-trained on a large corpus of text data by predicting the next word in a sentence given the previous context. GPT-2 has been used in a variety of applications, including chatbots, automated text summarization, and text completion.

\textbf{GPT-J-6B}~\citep{gpt-j} is a transformer model trained using Mesh Transformer JAX~\citep{mesh-transformer-jax}. It is a series of models with `6B' denoting 6 billion parameters.


\textbf{Flan-T5~\citep{raffel2020exploring,chung2022scaling}} Flan-T5 adopts a text-to-text strategy where input and output are both natural language sentences to execute a variety of tasks like machine translation, summarization, and question answering. This input-output form allows Flan-T5 to accomplish held-out tasks when given an input sentence as prompt.


% \textbf{T0~\citep{sanh2021multitask}} T0 tends to reach zero-shot generalization by mapping natural language tasks into a prompted form and convert a large set of supervised datasets into prompted datasets. These prompted datasets enables evaluating on held-out tasks.

\textbf{GPT-NEOX-20B~\citep{neox20b}} GPT-NeoX-20B is a language model with 20 billion parameters trained on the Pile. It is the largest public dense autoregressive model. It outperformed GPT-3 and FairSeq models with similar size in five-shot reasoning tasks.

\textbf{OPT~\citep{zhang2022opt}} Open Pre-trained Transformers (OPT) is a suite of pre-trained transformer models that are decoder-only and have parameter sizes ranging from 125 million to 175 billion. While offering comparable performance to GPT-3~\citep{brown2020language}, OPT-175B was developed with just 1/7th of the carbon footprint.

\textbf{BLOOM~\citep{scao2022bloom}} BLOOM extends pre-training from mono-lingual to cross-lingual. BLOOM combines one unsupervised objective and one supervised objective for pre-training. The unsupervised one only uses monolingual data, and the supervised one adopts parallel data. The cross-lingual language models can bring significant improvements for low-resource languages.

\textbf{text-davinci-002 and text-davinci-003} text-davinci-002 and text-davinci-003~\footnote{\url{https://platform.openai.com/docs/models/gpt-3}} are based on GPT-3~\citep{brown2020language}. They accomplish any task that other models can, generally produce output that is of higher quality, longer in length, and more faithful to instructions.

\section{Details on Prompts}
\label{append-promp}

\subsection{Prompts}
We list all prompts used in this study in \cref{tb-prompt}.

\begin{table}[htbp]
\caption{All prompts used in this study.}
\label{tb-prompt}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|p{12cm}}
\toprule
Dataset & Prompt \\ \midrule
SST-2 & {\ttfamily Please classify the following sentence into either positive or negative. Answer me with "positive" or "negative", just one word.} \\ \midrule
QQP & {\ttfamily Are the following two questions equivalent or not? Answer me with "equivalent" or "not\_equivalent".} \\ \midrule
MNLI & {\ttfamily Are the following two sentences entailment, neutral or contradiction? Answer me with "entailment", "neutral" or "contradiction".} \\ \midrule
QNLI & {\ttfamily Are the following question and sentence entailment or not\_entailment? Answer me with "entailment" or "not\_entailment".} \\ \midrule
RTE & {\ttfamily Are the following two sentences entailment or not\_entailment? Answer me with "entailment" or "not\_entailment".} \\ \midrule
AdvGLUE-T & {\ttfamily Translate the following sentence from Engilish to Chinese.} \\ \midrule
ANLI & {\ttfamily Are the following paragraph entailment, neutral or contradiction? Answer me with "entailment", "neutral" or "contradiction". The answer should be a single word. The answer is:} \\ \midrule
\flip & {\ttfamily Is the following sentence positive, neutral, or negative? Answer me with "positive", "neutral", or "negative", just one word.} \\ \midrule
\ddx & {\ttfamily Imagine you are an intern doctor. Based on the previous dialogue, what is the diagnosis? Select one answer among the following lists: {[}'spontaneous pneumothorax', 'cluster headache', 'boerhaave', 'spontaneous rib fracture', 'gerd', 'hiv (initial infection)', 'anemia', 'viral pharyngitis', 'inguinal hernia', 'myasthenia gravis', 'whooping cough', 'anaphylaxis', 'epiglottitis', 'guillain-barré syndrome', 'acute laryngitis', 'croup', 'psvt', 'atrial fibrillation', 'bronchiectasis', 'allergic sinusitis', 'chagas', 'scombroid food poisoning', 'myocarditis', 'larygospasm', 'acute dystonic reactions', 'localized edema', 'sle', 'tuberculosis', 'unstable angina', 'stable angina', 'ebola', 'acute otitis media', 'panic attack', 'bronchospasm / acute asthma exacerbation', 'bronchitis', 'acute copd exacerbation / infection', 'pulmonary embolism', 'urti', 'influenza', 'pneumonia', 'acute rhinosinusitis', 'chronic rhinosinusitis', 'bronchiolitis', 'pulmonary neoplasm', 'possible nstemi / stemi', 'sarcoidosis', 'pancreatic neoplasm', 'acute pulmonary edema', 'pericarditis', 'cannot decide'{]}. The answer should be a single word. The answer is:} \\ \bottomrule
\end{tabular}
}
\end{table}

\subsection{More Cases of Applying CoT}
We put more cases of applying CoT in Table~\ref{tab-more-cot-cases-1} and Table~\ref{tab-more-cot-cases-2}.

\begin{table}[!ht]
    \centering
    \caption{Cases of prompting text-davinci-003 with and without CoT on the QQP task.}
    \label{tab-more-cot-cases-1}
    \begin{tabular}{p{0.1\textwidth}|p{0.1\textwidth}|p{0.1\textwidth}|p{0.1\textwidth}|p{0.5\textwidth}}
    \toprule
        Question 1 & Question 2 & Ground Truth & Detailed Prompt & CoT Prompt \\ \midrule
        are alien realistic or are they fake ?  & Do aliens exists ? & equivalent & not equivalent & {\ttfamily the first question is asking whether aliens are real or not, while the second question is asking whether aliens exist or not. both questions are asking the same thing, so they are semantically equivalent. label: <equivalent> } \\ \midrule
         How c an I create the most popular question on Quora? & Which are the most popular questions on Quora presently that also create the most discussions? & not equivalent & equivalent & {\ttfamily first, we need to compare the two questions to see if they are asking the same thing. the first question is asking how to create the most popular question on quora, while the second question is asking which are the most popular questions on quora that create the most discussions. we can see that the two questions are asking about the same topic, but the first question is asking how to do something, while the second question is asking for a list of the most popular questions. therefore, the two questions are not semantically equivalent. label: <not equivalent>} \\ \midrule
         How can I creae the most popular question on Quora?  & Which are the most popular questions on Quora presently that also create the most discussions? & not equivalent & equivalent & {\ttfamily we can compare the two questions by looking at the keywords. both questions are asking about the most popular questions on quora. the first question is asking how to create the most popular question, while the second question is asking which questions are the most popular and create the most discussions. therefore, the two questions are related but not semantically equivalent. label: <not equivalent>} \\ \bottomrule
        % What was the deadliest battle in history?   & What was the bloodest bttle in histroy? & equivalent & not equivalent & first, we can compare the two questions and see that the only difference is the word "deadliest" and "bloodest". we can assume that these two words are synonyms and therefore the two questions are semantically equivalent. label: <equivalent> \\ \hline
    \end{tabular}
\end{table}

\begin{table}[!ht]
    \centering
    \caption{Cases of prompting text-davinci-003 with and without CoT on the QQP task (Cont.).}
    \label{tab-more-cot-cases-2}
    \begin{tabular}{p{0.1\textwidth}|p{0.1\textwidth}|p{0.1\textwidth}|p{0.1\textwidth}|p{0.5\textwidth}}
    \toprule
        Question 1 & Question 2 & Ground Truth & Detailed Prompt & CoT Prompt \\ \midrule
         What are the best things to do in Hog Kong?  & What is the best thing in Hong Kong? & equivalent & equivalent & {\ttfamily we can compare the two questions and see if they are asking the same thing. the first question is asking for a list of activities, while the second question is asking for a single activity. therefore, the two questions are not semantically equivalent. label: <not equivalent>} \\ \midrule
        % How do I buy used car in India?   & Whi ch used car should I buy in India? & not equivalent & not equivalent & we can compare the two questions by looking at the keywords. the first question is asking about how to buy a used car in india, while the second question is asking which used car to buy in india. both questions are asking about used cars in india, so they are semantically equivalent. label: <equivalent> \\ \hline
        Will consuming only eat dinner dinner tip to fitness loss ?  & Does eating dinner earlier in the evening help with weight loss ? & not equivalent & not equivalent & {\ttfamily we can compare the two questions by looking at the keywords. both questions are asking about the relationship between eating dinner and weight loss. the only difference is that the first question is asking if consuming only dinner will help with weight loss, while the second question is asking if eating dinner earlier in the evening will help with weight loss. therefore, the two questions are semantically equivalent. label: <equivalent>} \\ \midrule
        How can I build the most famous questions on Quora ? & Which are the most popular questions on Quora presently that also create the most discussions ? & not equivalent & equivalent & {\ttfamily first, we can compare the keywords in the two questions. both questions contain the words "quora", "questions", and "most". additionally, the first question contains the words "build" and "famous", while the second question contains the words "popular" and "create". this suggests that the two questions are asking about the same topic, but from different perspectives. therefore, the two questions are semantically equivalent. label: <equivalent> }\\ \bottomrule
    \end{tabular}
\end{table}

\subsection{OOD Case Study}
\label{append-oodexample}

We list some of the OOD examples for case study in \cref{tb-ood-example}.

\input{tables/tb-case-ood.tex}
